Variability-aware Datalog

Variability-aware computing is the efficient application of programs to different sets of inputs that exhibit some variability. One example is program analyses applied to Software Product Lines (SPLs). In this paper we present the design and development of a variability-aware version of the Souffl\'{e} Datalog engine. The engine can take facts annotated with Presence Conditions (PCs) as input, and compute the PCs of its inferred facts, eliminating facts that do not exist in any valid configuration. We evaluate our variability-aware Souffl\'{e} implementation on several fact sets annotated with PCs to measure the associated overhead in terms of processing time and database size.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}
\todo{intro}

==> synsem.tex <==
\section{Syntax and Semantics}
\label{sec:synsem}

\subsection{Syntax}

\begin{figure*}[t!]
	\centering
\begin{subfigure}[t]{0.49\textwidth}
	\centering
    \[
    \begin{array}{lcl}
    C &  = & \{\text{finite set of constant symbols}\}  \\
    V &  = & \{\text{finite set of variables}\}         \\
    P &  = & \{\text{finite set of predicate symbols}\}   \\
    \ldef{\featset} & \ldef{=} & \ldef{\{\text{finite set of features}\}} \\
    T & ::= & C~|~V \\
    L & ::= & P(T_1, ..., T_n)  \\
    F & ::= & P(C_1, ..., C_m)    \\
    R & ::= & L_0~\colonminus~L_1, ..., L_k \\
    \ldef{PC} & \ldef{::=} & \ldef{\true~|~\featset~|~\neg PC~|~PC \land PC} \\ 
    	      &            & \ldef{|~PC \lor PC} \\
    D & ::= & F~|~R~\ldef{|~F~@~PC~|~R~@~PC}
    \end{array}
    \]
    \vspace{-0.1in}
    \caption{Datalog syntax.}
    \label{fig:syntax}
\end{subfigure}
~
\begin{subfigure}[t]{0.49\textwidth}
	\centering
	\[
	\begin{array}{lcl}
	\assignment & : & V \to S \\
	\vars{C} 	& = & \{\text{variables in clause $D$}\} \\
	~[\assignment] D & = & D[v / \assignment(v)] \text{, for each free variable } \\ 
					 &   & v \text{ in } D \\
	\HB     	& = & \{p(c_1,...,c_n)~|~p \in P, c_1,...,c_n \in C\}	\\
	\cons{D}	& = & \{\text{logical consequences of clause $D$}\} \\
	\sym{$L_0 \colonminus L_1,...,L_k$} 	& = & \forall x_1,...,\forall x_m(L_1 \land ... \land L_k \implies L_0) \\
	&   & \vars{$L_0 \colonminus L_1, ..., L_k$}~=~\{x_1, ... , x_m\}	\\
	\end{array}
	\]
	\vspace{-0.1in}
	\caption{Datalog semantics.}
	\label{fig:semantics}
\end{subfigure}
\caption{Variability-aware Datalog syntax and semantics.}
\vspace{-0.1in}
\end{figure*}

Fig.~\ref{fig:syntax} defines the grammar of Datalog clauses as follows: (1)
building blocks are finite sets of constants, variables and predicate symbols;
(2) a \emph{term} is a constant or a variable symbol;
(3) a predicate expression is an $n$-ary predicate applied to arguments;% taking $n$ terms as arguments.
(4) a \term{fact} is a ground predicate expression, i.e., all of its arguments are constants;
(5) a \term{rule} is a Horn Clause of predicate expressions; and (6)
a \emph{Datalog clause} is either a fact or a rule.

We extend the standard grammar (extensions \ldef{highlighted}) of Datalog with \term{Presence Conditions(PCs)}. A PC is a propositional formula over a set of \term{features}. Each feature can be either present or absent in a configuration, so a PC actually denotes a set of possible configurations. Each Datalog clause has an associated PC, either explicitly specified using the '@' notation, or if left out the default PC is \true.

\subsection{Semantics}

Each clause is now annotated with a Presence Condition (PC). We refer to the annotated Inentional Database and annotated Extentional Database as $\liftedIDB$ and $\liftedEDB$. Given a configuration $\conf$, we define $\indexProd{\liftedEDB}{\conf}$ to be the set of facts from $\liftedEDB$ which only exist in the product set defined by $\conf$:
\[
\indexProd{\liftedEDB}{\conf} = \{f~|~(f, \pc{}) \in \liftedEDB \land \sat(\pc{} \land \conf)\}
\]


Fig.~\ref{fig:semantics} summarizes the semantics of Datalog, with variability-aware extensiones \ldef{highlighted} as follows:
(1) A value assignment $\assignment$ assigns values to variables;
(2) \vars{C} is the set of variables occuring in clause $D$;
(3) A variable substitution over clause $D$ using assignment $\assignment$ replaces each variable $v$ in $D$ with $\assignment(v)$;
(4) The Herbrand Base (\HB) is the set of all the possible facts that can be represented in the language;
(5) \cons{D} is the set of all facts that are logical consequences of clause $D$;
(6) The semantics of the clause $L_0~\colonminus~L_1, ..., L_k$ is the first-order formula $\forall x_1,...,\forall x_m(L_1 \land ... \land L_k \implies L_0)$, where all variables in the clause are universally quantified. Datalog inference is based on applying Modes Ponens to infer new facts from existing ones and rules.


\begin{figure}
	\centering
	\[
	\infer[\widehat{MP}]{([\assignment]C, \ldef{pc_r \wedge pc_1 \wedge ... \wedge pc_n})} {%
		(C \colonminus~\premise{1}, ..., \premise{n}, \ldef{pc_r})
		& [\assignment]\premise{1} = \fact{1}
		& ...
		& [\assignment]\premise{n} = \fact{n}
		& \forall(1 \leq i \leq n), (\fact{i}, \ldef{\pc{i}}) \in \liftedEDB
		& \assignment:V \to S
	}
	\]
	\caption{Modus Ponens for variability-aware Datalog clause inference}
	\label{fig:MPlifted}
\end{figure}

Fig.~\ref{fig:MPlifted} outlines the semantics of variability-aware Modus Ponens inference. Since each Datalog clause now has a PC, then any inferred clauses should also be assigned a PC. Intuitively, a conclusion exists only if all its premises, and the rule used in its inference, all exist. In other words, the set of worlds where the conclusion exists is the intersection of sets of worlds of each of the premises and the inference rule. This PC is denoted by the conjunction PCs of the premises together with the PC of the rule.

\section{Inference and Correctness}
\label{sec:inference}

The standard Datalog inference algorithm ($\resolve$) is a simple fixpoint loop that goes through each of the rules, checks if some facts in the $\EDB$ satisfy the premises, and if they do, the conclusion is added to the $\EDB$ if it does not already exist. This is repeated until no new facts can be inferred. Because the constant and predicate sets are finite, this algorithm is guaranteed to terminate in polynomial time in the number of input facts~\cite{Ceri:1989}.

Algorithm~\ref{alg:inference_lifted} is the variability-aware version of $\resolve$, called $\resolveLifted$. The main variability-aware extensions to the algorithm (\ldef{highlighted}) are:
(1) Each clause (a fact or a rule) has a PC;
(2) When a conclusion is inferred, its PC becomes the conjunction of the PC of the rule, the PCs of each of the premises, and also $\FM$ (to make sure facts stay within the set of valid world configurations);
(3) If that PC is not satisfiable, then it does not represent a set of valid configurations. In this case we can simply ignore it;
(4) If that conclusion already exists in $\liftedEDB$ with the same PC, then we can still ignore it because we have not inferred anything new;
(5) However, if the conclusion exists with a different PC (i.e. it belongs to another set of configurations), then we need to modify that PC to denote the union of the existing and new sets of configurations. This is achieved by disjoining the existing and new PCs.

Please note that the satisfiability check on the calculated PC makes the worst-case complexity of this algorithm exponential in the number of features. In practice though with tens of features modern satisfiability checkers and Binary Decision Diagram (BDD) packages can determine propositional satisfiability pretty efficiently. If the number of featuers is in the order of hundreds or more, we can disable this satisfiability check, on the expense of possibly adding facts that do not really belong to valid configurations to the database. This might grow the database size unnecessarily, but does not jeopordize the correctness of the algorithm. Removing those vacuous facts can be done as a post-processing step after inference is over.

\begin{algorithm}
    \caption{Lifted inference algorithm $\resolveLifted$.}
    \label{alg:inference_lifted}
    \SetAlgoLined
    \KwData{input: $\liftedIDB$, $\liftedEDB$}
    \KwResult{$\liftedEDB$ + annotated inferred clauses}
    \Repeat{fixpoint}
    {
        fixpoint = \true\;
        \ForEach
        {$(C$ \colonminus~$\premise{1}, ..., \premise{n}, \ldef{pc_r}) \in \liftedIDB$}
        {\ForEach{$(\assignment, (\fact{1}, \ldef{\pc{1}}),...,(\fact{n}, \ldef{\pc{n}})), (\fact{i}, \ldef{\pc{i}}) \in \liftedEDB, [\assignment]\premise{i} = \fact{i}$}
            {
                \ldef{$\pc{c} = pc_r \land \pc{1} \land ... \land \pc{n} \land \FM$}\;
                \If{\ldef{sat($\pc{c}$)}}
                {\If{$([\assignment]C, \ldef{\pc{c}}) \notin \liftedEDB$}
                    {
                        fixpoint = \false\;
                        \If{\ldef{$\exists \pc{d}, ([\assignment]C, \pc{d}) \in \liftedEDB$}}
                        {\ldef{$\pc{c} = \pc{c} \lor \pc{d}$\;
                                $\liftedEDB = \liftedEDB - \{([\assignment]C, \pc{d})\}$}}
                        \ldef{$\liftedEDB = \liftedEDB \cup \{[\assignment]C, \pc{c})\}$}}
                }
            }
        }
    }
    return $\liftedEDB$\;
\end{algorithm}

\subsection{Correctness Criteria}
When applying the lifted inference algorithm $\resolveLifted$ to a set of rules $IDB$ and a set of annotated facts $\liftedEDB$, we expect the result to be exactly the union of the results of applying $\resolve$ to facts from each product individually. Moreover, each clause in the result of $\resolveLifted$ has to be properly annotated (i.e., its presence condition has to represent exactly the set of products having this clause in their un-lifted  analysis results).
%This is formally specified in Theorem~\ref{th:correctness}.
\begin{theorem}
    Given a set of features $\featset$, a set of PC-annotated rules $liftedIDB$, and a set of PC-annotated facts $\liftedEDB$:
    \[
    \forall (\conf \in \Conf(\featset)), \indexProd{\resolveLifted(\liftedEDB)}{\conf} = \resolve(\indexProd{\liftedEDB}{\conf})
    \]
    \label{th:correctness}
\end{theorem}

\begin{proof}
    Set equality is equivalent to a double-implication of mutual set containment, so we need to prove the implication in both directions:
    \begin{itemize}
        \item $C \in \indexProd{\resolveLifted(\liftedEDB)}{\conf} \implies C \in \resolve(\indexProd{\liftedEDB}{\conf})$ \\
        By structural induction over the derivation tree of $C$: \\
        \basecase $(C, \pc{}) \in \liftedEDB$, where $\sat(\pc{} \land \conf)$. Then $C \in \indexProd{\liftedEDB}{\conf}$ (by definition of restriction operator). Since
        inputs are already included in the output of $\resolve$, $C \in \resolve(\indexProd{\liftedEDB}{\conf})$. \\
        \indhypo Given a rule $R = C~\text{\colonminus}~\premise{1}, ..., \premise{n}$, and a variable assignment $\assignment$,
        \[ \forall(1 \leq i \leq n):[\assignment]\premise{i} \in \indexProd{\resolveLifted(\liftedEDB)}{\conf} \implies [\assignment]\premise{i} \in \resolve(\indexProd{\liftedEDB}{\conf}) \]
        
        \indstep $C$ is derived by $\widehat{MP}$ (Fig.~\ref{fig:MPlifted}) from rule $R$. Since all the premises of $C$ are in $\resolve(\indexProd{\liftedEDB}{\conf})$ (induction hypothesis), then so is $C$ ($MP$).
        \item $C \in \resolve(\indexProd{\liftedEDB}{\conf}) \implies C \in \indexProd{\resolveLifted(\liftedEDB)}{\conf}$ \\
        By structural induction over the derivation tree of $C$: \\
        \basecase Assume $(C, \pc{}) \in \liftedEDB$, for some $\pc{}$, where $\sat(\pc{} \land \conf)$. Then $(C,pc) \in \resolveLifted(\liftedEDB)$ (input included in output of $\resolveLifted$). Since $\pc{} \land \conf$ is satisfiable, then $C \in \indexProd{\resolveLifted(\liftedEDB)}{\conf}$ (definition of restriction).\\
        \indhypo Given a rule $R = C~\text{\colonminus}~\premise{1}, ..., \premise{n}$, and a variable assignment $\assignment$,
        \[ \forall(1 \leq i \leq n):[\assignment]\premise{i} \in \resolve(\indexProd{\liftedEDB}{\conf}) \implies [\assignment]\premise{i} \in \indexProd{\resolveLifted(\liftedEDB)}{\conf} \]
        \indstep $C$ is derived by $MP$ (Fig.~\ref{fig:MPlifted}) from rule $R$. Since all the premises of $C$ are in $\indexProd{\resolveLifted(\liftedEDB)}{\conf}$ (induction hypothesis), then so is $C$ ($\widehat{MP}$).
    \end{itemize}
\end{proof}
